Practical Speech Re-use Prevention in Voice-driven Services

Voice-driven services (VDS) are being used in a variety of applications ranging from smart home control to payments using digital assistants. The input to such services is often captured via an open voice channel, e.g., using a microphone, in an unsupervised setting. One of the key operational security requirements in such setting is the freshness of the input speech. We present AEOLUS, a security overlay that proactively embeds a dynamic acoustic nonce at the time of user interaction, and detects the presence of the embedded nonce in the recorded speech to ensure freshness. We demonstrate that acoustic nonce can (i) be reliably embedded and retrieved, and (ii) be non-disruptive (and even imperceptible) to a VDS user. Optimal parameters (acoustic nonce's operating frequency, amplitude, and bitrate) are determined for (i) and (ii) from a practical perspective. Experimental results show that AEOLUS yields 0.5% FRR at 0% FAR for speech re-use prevention upto a distance of 4 meters in three real-world environments with different background noise levels. We also conduct a user study with 120 participants, which shows that the acoustic nonce does not degrade overall user experience for 94.16% of speech samples, on average, in these environments. AEOLUS can therefore be used in practice to prevent speech re-use and ensure the freshness of speech input.

==> sections/background.tex <==
\section{Background and Related Work}

In this section, we 


%In this section, we cover some backgrounds related to voice assistant security. First, we talk about replay attacks and the current defense strategies. Second, we present speaker recognition (a.k.a. voice authentication) used in critical voice-based functionalities such as voice shopping. Third, we illustrate the nonce-based authentication scheme that is relevant to our work. 

%MSH avoid using Wikipedia text or image, and I like the figure here better: https://www.researchgate.net/publication/224245051_Nested_mechanism_for_mutual_authentication/figures?lo=1




%MSH we should decide VUI, voice-enable or voice-controlled, use the same throughout the document.

VCS \cite{vui} is operated by voice commands, as shown in Figure \ref{fig:firstarch}. Users' voice commands are transcribed and comprehended by the system and the proper response is returned either by playing a verbal response  (e.g., announcing the time) or taking an external action (e.g., turning lights on/off).
The system is triggered by a wake-up command (e.g., Alexa, Hey Siri) and then it works in a turn-taking mode, the device is idle while the user sends commands and the user usually is silent when the device plays responses. \tool\ leverages device idle time to embed the acoustic nonce. 

VCS works in four stages, 1) a voice channel over which the verbal requests and responses are exchanged, 2) the text/speech processing engine to convert speech-to-text and text-to-speech, and 3) speaker verification to recognize the user for penalization or security purposes and 4) the text/intent processing engine to execute commands.  Our goal is to protect the voice channel against replay attacks. 



\subsection{Speaker Recognition}
 Voice or speaker recognition analyzes a person's voice to verify their identity. Airways and soft-tissue cavities, as well as the shape and movement of the mouth and jaw, influence voice patterns to create a unique voiceprint. 
 %MSH next can be removed
 Speaker recognition is a type of voice recognition technology. However, it is not the same as speech recognition, which is the technology used in speech-to-text applications. Speech recognition can make sense of verbal language, but it cannot verify the identity of the speaker based on his or her unique vocal attributes; speaker verification can. 
 Voice biometrics is still in the early stages of development and is the target of different attacks such as replay attacks and voice synthesis attacks. 
 
 Replay attacks are known to be the most accessible attack~\cite{pindrop} to affect a VCS. It requires only a simple microphone and loudspeaker to launch effective attacks. In this attack, the attacker records the target user when s/he speaks a command in a hope to replay the command in the future and gain access to the system. Speaker verification deployed in current systems fail to detect such attack since the attacked voice sample captures the exact feature of the target user. 
Several defense techniques such as liveness detection are proposed to detect replay attacks \cite{zhang2017hearing, shiota2015voice}.  However, these techniques have distance or hardware limitations, and therefore, are not practical as shown by recent studies  \cite{shirvanian2019quantifying}. 


 Voice synthesis attacks are another possible attack on speaker recognition. Voice conversion and speech synthesis tools try to generate an individual's voice by mimicking characteristics of the target speaker. To generate a convincing voice that can break a robust speaker recognition system, many speech synthesis tools require a collection of the target voice and several hours of training. Research in the speaker recognition domain is advancing to detect this type of attack. A collection of work in this area can be found in the recent ASVSPoof 2019 challenge \cite{todisco2019asvspoof}. 

\subsection{Nonce-based Authentication}
 In the security domain, a nonce is often a random or pseudo-random number issued in an authentication protocol to ensure that earlier messages are not reused in a replay attempt, as shown in Figure~\ref{fig:nonce}. For each authentication request-response session, the server assigns and transfers a fresh nonce as a request and expects to receive a response from the client that contains the nonce along with the authentication credential. The idea is that an attacker who has eavesdropped previous communications cannot resubmit the response since a freshly generated request contains a nonce not available in earlier authentications.
 The nonce and the credential are bundled and encrypted as a single message to avoid the removal of nonce and access to the encrypted credential. 
 

\tool{'s} strategy uses a similar concept, however, unlike communications happening between two machines over the data channel, an acoustic nonce cannot be simply encrypted or hashed. Therefore, we propose a voice frequency-range hopping technique to embed the acoustic nonce. This embedding works similar to encrypting the bundle of nonce and credential in traditional nonce authentication.  





%\subsection{Voice Controlled Systems}


\begin{figure}[t]
\centering
  \includegraphics[width=1\linewidth]{figures/background1.pdf}
%\vspace{-0.2in}
  \caption{Nonce-based Authentication}
  \label{fig:nonce}
\end{figure}
\begin{figure*}
\centering
  \includegraphics[width=0.8\linewidth]{figures/overview1.pdf}
%\vspace{-0.2in}
  \caption{\tool\ in VCS.}
  \label{fig:overview1}
\end{figure*}

==> sections/design1.tex <==

%%MSH 27/01 I think we need one for the accuracy of the technique and one for robustness, so detecting previous attack comes under accuracy


\section{Voice Frequency-hopping Spread Spectrum (VFHSS)}
\label{sec:vfhss}
\begin{comment}
\begin{figure}[b]
\centering
  \includegraphics[width=0.8\linewidth]{figures/vfhss.pdf}
%\vspace{-0.2in}
  \caption{Example VFHSS consists of four waves in different frequencies. }
  \label{fig:vfhss}
\end{figure}
\end{comment}
To establish a systematic approach for tackling the challenges, we first model the questions with a convex maximization problem. 

%\textbf{Design Goal.} 
In our setting, an attacker's goal is to remove the nonce from the recorded speech. The attack is considered to be successful if a clean audio record without any detectable nonce residual can be produced. 
%This leads to two causally-related design goals. In here, 
This clean audio record should also be able to pass speaker verification and other VCS functionalities.  First, \tool\ should detect the existence of previously embedded nonce fully or partially. Second, the embedded nonce can be preserved, partially or fully, when different watermark attacks are performed.

%\textbf{What are watermark attacks?} 
\smallskip\noindent\textbf{Watermark Attacks.}
There are three major types of watermark attacks that are relevant to our work ~\cite{arnold2003techniques}: detection of watermark, embedding of watermark and removal of watermark. As described earlier we focus on addressing the threats from removal attacks. We list common watermark removal attacks in the following, note that some of these techniques are also used in popular noise cancellation:




\begin{itemize}[noitemsep,leftmargin=*]
    \item Resampling. In digital recording, sampling process takes snapshots of an audio or video. For example, a popular sampling rate for audio is 44.1kHz. Attacks may sample the audio in a different frequency to remove sampling-dependent watermark.
    \item Amplitude Compression. Attackers may resize the amplitude of audio signals recorded to avoid amplitude-related watermark detection.
    %\item Time Scale Modification. This attack typically speeds up or slows down a sound without affecting the frequency content.
    \item Filtering. Filtering is effective in removing audio signals from a specific range of frequency. For example, %DolphinAttack and other 
    ultrasound-based inaudible voice commands can be removed by applying Low Pass Filter to separate audio signals from inaudible frequencies.  
    \item Lossy Compression. This attack leverages data encoding methods that uses inexact approximations and partial data discarding to represent the audio. For example, MP3~\cite{mp3}, or MPEG-1 Audio Layer III, conducts audio file size reduction by taking advantage of a perceptual limitation of human hearing.
    \item Equalization. This process commonly used to alter the frequency response of an audio system using linear filters. A frequency response is a measure the audio output as a function of frequency, in comparison to the input. For example, a 5kHz wave input may have a 4kHz response as the output.
    \item Additive Noise. An attack could add noise to decrease SNR (signal-to-noise) ratio so that watermark signals cannot be extracted successfully.
\end{itemize}


\smallskip\noindent\textbf{Resistance to Watermark Removal.} 
To address the issue of removable watermarking, as shown in Figure~\ref{fig:vfhss}, we leverage Frequency-hopping Spread Spectrum (FHSS)~\cite{cvejic2004spread,cvejic2004algorithms} to obtain high robustness
against standard watermark attacks.

%We propose to use FHSS to provide the rubostness against watermark removal attacks. 
Although is is known that FHSS prevents attacks from getting useful clean audio recording, we also argue it is only useful in voice frequency range because filtering attack could easily filter out high frequency signal.
In practice, a frequency drifting is commonly observed in real-world acoustic wave transmission. This is because of the hardware limitation such as the vibration sensitivity of a loud speaker.  

%MSH I cannot find the connection between the next two items with this section, can you connect them to the team of this subsection? If these two are related to integrity goal move it to previous section



%\smallskip\noindent\textbf{Multi-band Acoustic Tagging.} 
%We f that the transmission rate of acoustic communication is limited. 
In our preliminary tests, we  noticed that the transmission rate of acoustic communication is limited as we could reach at most 20 bits/sec in the close distance (i.e., within 5 meter) transmission. As a result, we propose to leverage \textit{\textbf{multi-band acoustic tagging}}. This means \tool\ will use not only one range of frequency for nonce transmission. Multiple bands are used, for example, as shown in Figure~\ref{fig:spectro1}, two bands are used either with or without frequency hopping. Note that, the frequency hopping starts at 0.5 seconds. 


\begin{figure}[h]
\centering
  \includegraphics[width=0.90\linewidth]{figures/spectro1.pdf}
\vspace{-2mm}
  \caption{Spectrogram of an Example Multi-band Acoustic Nonce.}
  \label{fig:spectro1}
\end{figure}

==> sections/design2.tex <==


\begin{table}[h]
\centering
\footnotesize
\vspace{-0mm}
\caption{Example of Decibel Level Reference~\cite{yaledecibel}}
\vspace{-0mm}
\label{table:decibel}
\begin{tabular}{ll}
\toprule[1.5pt]
Environmental Noise & \parbox[t]{1.2cm}{dBA \textdagger}\\
\midrule
Subway train at 200'  & 95\\
Level at which sustained exposure           & \multirow{ 2}{*}{80-90}\\
may result in hearing
loss& \\
City Traffic & 85\\
Telephone dial tone    &  80   \&\\

Chamber music, in a small auditorium  & 75-85 \\
Vacuum cleaner         & 75\\

Normal conversation     &  60-70 \\

Business Office   & 60-65 \\

Household refrigerator   &55\\

Suburban area at night   & 40\\

Quiet natural area with no wind & 20\\

    \bottomrule
\end{tabular}
\begin{tablenotes}
\centering
\item \textdagger: dBA = Decibels, A weighted 
\end{tablenotes}
\end{table}


%%%MSH 04/07 CCS: Move the table and figure 7 to appendix, and add a summary of the two in the text citing the three papers. 


==> sections/implementation.tex <==

%%%MSH 04/07 evaluation supports the design goal and name the section  experimental setup 
%%MSH 04/13 we can also have one section for simulation, and one section for real world, setup and results
\section{Experiment Setup}

\begin{comment}
\smallskip \noindent \textbf{Audio Watermark Removal.} As discussed in Section~\ref{sec:vfhss}, we aim to test \tool\ with 6 common audio watermark removal techniques. All these techniques are implemented using Matlab which has many audio signal processing libraries such as Audio Toolbox, Wavelet Toolbox.

\smallskip \noindent \textbf{Speaker Recognition.} We use Microsoft Speaker Recognition system~\cite{ms_speaker} as the target testing function. To remove human factors in this test, we use synthesized speech with Amazon Polly~\cite{polly} as the voice input to enroll a speaker profile. Then the same synthesis scheme is used to generate testing speech to test with the profile identification system. 





Two types of simulation are conducted in this work. 

\smallskip \noindent \textbf{MCRoomSim.}
First, to evaluate how different parameters affect encoded the propagation of acoustic waves in a room, we leverage a Matlab-based library, MCRoomSim~\cite{wabnitz2010room}. 
While Acoustic Communication Kit provides transmitter and receiver parts of \tool, we also simulate how acoustic waves propagate in the indoor environment. MCRoomSim allows \tool\ to be tested exclusively before the real-world experiments. In MCRoomSim, various physical environment parameters are set to qualitatively test \tool. For example, one can adjust the room size, air absorption, etc. 

%%MSH 04/13/ explain the dataset, show that it is extensive, thousands of users


==> sections/related.tex <==
\section{Related Work}

%In this section, we discuss defense techniques that are relevant to prevent replay attacks. 

%MSH Are these not liveness detection? shouldn't we have one subsection for liveness detection? I think two factor authentication is not relavant here but liveness detection is  
\noindent\textbf{Two Factor Authentication}
% the mobicom paper
One effective way of authenticating an insecure channel is to use secured factors to assist the authentication process. For example, text messages are used to prove users' identity in online banking, shopping, etc. In voice channel authentication aspect, Feng et al.~\cite{feng2017continuous} presents a method to authenticate a human speaker with extra sensors that collect  body-surface vibrations. 
Another way of preventing replay attacks is to identify the loud speakers used in attacking voice channel~\cite{chen2017you}. In specific, the magnetic field incurred by using loud speakers are used to detect replay attacks. However, this technique works only in very close range (within 8 centimeter). 
Due to these limitations, these techniques are not practical enough for real-world deployment, and hence, are not  used in popular VCS. In this work, we aim to design a defense solution that works in a reasonable range without extra devices needed.

\noindent\textbf{Challenge-response Authentication.}
% session key usage, and two party model
% it is used to detect replay attacks, giving the insight of using session key
%MSH: any paper in this scope? Maybe FIDO?
Challenge-response protocols are used to mitigate replay attacks in authentication over data channel. In this approach, typically, a randomly generated key (either public or private) is used for authentication. However, in the setting of using voice assists, such shared keys between a human user and VCS does not exist. Our mitigation, essentially uses the concept of challenge-response authentication in the data communication and applies it in the context of open voice channel to prevent replay attack. 


\noindent\textbf{Audio Passphrases.}
VCS users might authenticate using a predefined passphrase even when speaker recognition is not incorporated. However, this passphrase is spoken in an open voice channel and not an encrypted data channel. Once the attacker eavesdrops the passphrase s/he could replay it in future. Our mitigation can even protect replay of passphrases similar to the way nonce authentication protects replay of authentication credentials.  

\noindent\textbf{Audio Watermarking Techniques.}
% old papers, and clarify the difference
%MSH Give some information about these papers
Traditional digital audio watermarking techniques have already been studied in~\cite{swanson1998robust}~\cite{bassia2001robust}. The fundamental differences between our work and watermarking techniques are three-folded. First, we work with a real-time system rather than an existing audio files. Therefore, our system needs to work in real-time with various audio length and content. Second, we work with open voice channels and not an offline audio file, and therefore, it is not as simple as mixing the audio watermarking with an audio file offline. Third, the main goal of previous audio watermarking is to provide copyright protection, while we mainly aim to prevent replay attacks. Hence, the embedded information should be dynamic in our technique, unlike a static copyright information embedded in an audio file. 

\smallskip\noindent\textbf{Voice-driven Customer Service}
Voiceprint-based speaker recognition is being used to verify the identity of customers. For example, Citi Bank launched voiceprint-based authentication in 2016~\cite{citivoiceprint}. Within the first year itself, over 1 million customers used the service in Asia Pacific region. Like voice-based payments, voice-driven customer service is susceptible to speech re-use for authenticate. 

